Understanding Design Fixation in Generative AI

Generative AI (GenAI) provides new opportunities for creativity support, but the phenomenon of GenAI design fixation remains underexplored. While human design fixation typically constrains ideas to familiar or existing solutions, our findings reveal that GenAI similarly experience design fixation, limiting its ability to generate novel and diverse design outcomes. To advance understanding of GenAI design fixation, we propose a theoretical framework includes the definition, causes, manifestations, and impacts of GenAI design fixation for creative design. We also conducted an experimental study to investigate the characteristics of GenAI design fixation in practice. We summarize how GenAI design fixation manifests in text generation model and image generation model respectively. Furthermore, we propose methods for mitigating GenAI design fixation for future creativity support tool design. We recommend adopting the lens of GenAI design fixation for creativity-oriented HCI research, as the unique perspectives and insights it provides.

==> sections/appen.tex <==
%椅子设计相关words的词频分析
\begin{table}[ht]
\centering
\caption{Comparison of frequency of references to chair design keywords in design solutions in Red dot and ChatGPT, normalized per 100 cases.}
\label{tab:chair_parts_comparison}
\begin{tabularx}{0.4\textwidth}{Xrr}
\toprule
\textbf{Part} & \textbf{Red dot (per 100)} & \textbf{ChatGPT (per 100)} \\
\midrule
Seat          & \calc{70}{105}             & \calc{44}{96}                   \\
Leg           & \calc{49}{105}             & \calc{10}{96}                   \\
Backrest      & \calc{29}{105}             & \calc{33}{96}                   \\
Frame         & \calc{23}{105}             & \calc{9}{96}                    \\
Base          & \calc{22}{105}             & \calc{11}{96}                   \\
Armrest       & \calc{15}{105}             & \calc{14}{96}                   \\
Cushion       & \calc{7}{105}              & \calc{9}{96}                    \\
Footrest      & \calc{2}{105}              & \calc{5}{96}                    \\
Headrest      & \calc{2}{105}              & \calc{2}{96}                    \\
\midrule
\textbf{Total} & \textbf{\calc{219}{105}}  & \textbf{\calc{137}{96}}         \\
\bottomrule
\end{tabularx}
\end{table}
